A Unified Framework for Continual Learning and Unlearning

Continual learning and machine unlearning are crucial challenges in machine learning, typically addressed separately. Continual learning focuses on adapting to new knowledge while preserving past information, whereas unlearning involves selectively forgetting specific subsets of data. In this paper, we introduce a new framework that jointly tackles both tasks by leveraging controlled knowledge distillation. Our approach enables efficient learning with minimal forgetting and effective targeted unlearning. By incorporating a fixed memory buffer, the system supports learning new concepts while retaining prior knowledge. The distillation process is carefully managed to ensure a balance between acquiring new information and forgetting specific data as needed. Experimental results on benchmark datasets show that our method matches or exceeds the performance of existing approaches in both continual learning and machine unlearning. This unified framework is the first to address both challenges simultaneously, paving the way for adaptable models capable of dynamic learning and forgetting while maintaining strong overall performance. Source code: \textcolor{blue}{https://respailab.github.io/CLMUL}

==> sec/X_aaai_Reproducibility_Checklist.tex <==
\newpage

\section*{Reproducibility Checklist}

\begin{enumerate}
    \item Includes a conceptual outline and/or pseudocode description of AI methods introduced
    \begin{itemize}
        \item [] \textbf{(X)} Yes
        \item [] \textbf{( )} Partial
        \item [] \textbf{( )} No
        \item [] \textbf{( )} N/A
    \end{itemize}

    \item Clearly delineates statements that are opinions, hypothesis, and speculation from objective facts and results
    \begin{itemize}
        \item [] \textbf{(X)} Yes
        \item [] \textbf{( )} No
    \end{itemize}

    \item Provides well marked pedagogical references for less-familiar readers to gain background necessary to replicate the paper
    \begin{itemize}
        \item [] \textbf{(X)} Yes
        \item [] \textbf{( )} No
    \end{itemize}

    \item Does this paper make theoretical contributions?
    \begin{itemize}
        \item [] \textbf{( )} Yes
        \item [] \textbf{(X)} No
    \end{itemize}

    \item[] If yes, please complete the list below.
    \begin{enumerate}
        \item All assumptions and restrictions are stated clearly and formally.
        \begin{itemize}
            \item [] \textbf{( )} Yes
            \item [] \textbf{( )} Partial
            \item [] \textbf{( )} No
            \item [] \textbf{(X)} N/A
        \end{itemize}
        \item All novel claims are stated formally (e.g., in theorem statements).
        \begin{itemize}
            \item [] \textbf{( )} Yes
            \item [] \textbf{( )} Partial
            \item [] \textbf{( )} No
            \item [] \textbf{(X)} N/A
        \end{itemize}
        \item Proofs of all novel claims are included.
        \begin{itemize}
            \item [] \textbf{( )} Yes
            \item [] \textbf{( )} Partial
            \item [] \textbf{( )} No
            \item [] \textbf{(X)} N/A
        \end{itemize}
        \item Proof sketches or intuitions are given for complex and/or novel results.
        \begin{itemize}
            \item [] \textbf{(X)} Yes
            \item [] \textbf{( )} Partial
            \item [] \textbf{( )} No
            \item [] \textbf{()} N/A
        \end{itemize}
        \item Appropriate citations to theoretical tools used are given.
        \begin{itemize}
            \item [] \textbf{( )} Yes
            \item [] \textbf{( )} No
            \item [] \textbf{(X)} N/A
        \end{itemize}
        \item All theoretical claims are demonstrated empirically to hold.
        \begin{itemize}
            \item [] \textbf{(X)} Yes
            \item [] \textbf{( )} Partial
            \item [] \textbf{( )} No
            \item [] \textbf{()} N/A
        \end{itemize}
        \item All experimental code used to eliminate or disprove claims is included.
        \begin{itemize}
            \item [] \textbf{( )} Yes
            \item [] \textbf{( )} No
            \item [] \textbf{(X)} N/A
        \end{itemize}
    \end{enumerate}

    \item Does this paper rely on one or more datasets?
    \begin{itemize}
        \item [] \textbf{(X)} Yes
        \item [] \textbf{( )} No
    \end{itemize}

    \item[] If yes, please complete the list below.
    \begin{enumerate}
        \item A motivation is given for why the experiments are conducted on the selected datasets.
        \begin{itemize}
            \item [] \textbf{(X)} Yes
            \item [] \textbf{( )} Partial
            \item [] \textbf{( )} No
            \item [] \textbf{( )} N/A
        \end{itemize}
        \item All novel datasets introduced in this paper are included in a data appendix.
        \begin{itemize}
            \item [] \textbf{( )} Yes
            \item [] \textbf{( )} Partial
            \item [] \textbf{( )} No
            \item [] \textbf{(X)} N/A
        \end{itemize}
        \item All novel datasets introduced in this paper will be made publicly available upon publication of the paper with a license that allows free usage for research purposes.
        \begin{itemize}
            \item [] \textbf{( )} Yes
            \item [] \textbf{( )} Partial
            \item [] \textbf{( )} No
            \item [] \textbf{(X)} N/A
        \end{itemize}
        \item All datasets drawn from the existing literature (potentially including authors’ own previously published work) are accompanied by appropriate citations.
        \begin{itemize}
            \item [] \textbf{(X)} Yes
            \item [] \textbf{( )} No
            \item [] \textbf{( )} N/A
        \end{itemize}
        \item All datasets drawn from the existing literature (potentially including authors’ own previously published work) are publicly available.
        \begin{itemize}
            \item [] \textbf{(X)} Yes
            \item [] \textbf{( )} Partial
            \item [] \textbf{( )} No
            \item [] \textbf{( )} N/A
        \end{itemize}
        \item All datasets that are not publicly available are described in detail, with explanation why publicly available alternatives are not scientifically satisficing.
        \begin{itemize}
            \item [] \textbf{( )} Yes
            \item [] \textbf{( )} Partial
            \item [] \textbf{( )} No
            \item [] \textbf{(X)} N/A
        \end{itemize}
    \end{enumerate}

    \item Does this paper include computational experiments?
    \begin{itemize}
        \item [] \textbf{(X)} Yes
        \item [] \textbf{( )} No
    \end{itemize}

    \item[] If yes, please complete the list below.
    \begin{enumerate}
        \item Any code required for pre-processing data is included in the appendix.
        \begin{itemize}
            \item [] \textbf{( )} Yes
            \item [] \textbf{( )} Partial
            \item [] \textbf{(X)} No
            \item [] Code will be released after review, if the paper is accepted.
        \end{itemize}
        \item All source code required for conducting and analyzing the experiments is included in a code appendix.
        \begin{itemize}
            \item [] \textbf{( )} Yes
            \item [] \textbf{( )} Partial
            \item [] \textbf{(X)} No
            \item [] Code will be released after review, if the paper is accepted.
        \end{itemize}
        \item All source code required for conducting and analyzing the experiments will be made publicly available upon publication of the paper with a license that allows free usage for research purposes.
        \begin{itemize}
            \item [] \textbf{(X )} Yes
            \item [] \textbf{( )} Partial
            \item [] \textbf{()} No
            \item [] Code will be released after review, if the paper is accepted.
        \end{itemize}
        \item All source code implementing new methods have comments detailing the implementation, with references to the paper where each step comes from.
        \begin{itemize}
            \item [] \textbf{(X )} Yes
            \item [] \textbf{( )} Partial
            \item [] \textbf{()} No
            \item [] Code will be released after review, if the paper is accepted.
        \end{itemize}
        \item If an algorithm depends on randomness, then the method used for setting seeds is described in a way sufficient to allow replication of results.
        \begin{itemize}
            \item [] \textbf{(X)} Yes
            \item [] \textbf{( )} Partial
            \item [] \textbf{( )} No
            \item [] \textbf{( )} N/A

        \end{itemize}
        \item This paper specifies the computing infrastructure used for running experiments (hardware and software), including GPU/CPU models; amount of memory; operating system; names and versions of relevant software libraries and frameworks.
        \begin{itemize}
            \item [] \textbf{(X)} Yes
            \item [] \textbf{( )} Partial
            \item [] \textbf{( )} No

        \end{itemize}
        \item This paper formally describes evaluation metrics used and explains the motivation for choosing these metrics.
        \begin{itemize}
            \item [] \textbf{(X)} Yes
            \item [] \textbf{( )} Partial
            \item [] \textbf{( )} No
        
        \end{itemize}
        \item This paper states the number of algorithm runs used to compute each reported result.
        \begin{itemize}
            \item [] \textbf{(X)} Yes
            \item [] \textbf{( )} No
      \ref{sec:exp}.
        \end{itemize}
        \item Analysis of experiments goes beyond single-dimensional summaries of performance (e.g., average; median) to include measures of variation, confidence, or other distributional information.
        \begin{itemize}
            \item [] \textbf{(X)} Yes
            \item [] \textbf{( )} No
            
        \end{itemize}
        \item The significance of any improvement or decrease in performance is judged using appropriate statistical tests (e.g., Wilcoxon signed-rank).
        \begin{itemize}
            \item [] \textbf{(X)} Yes
            \item [] \textbf{( )} Partial
            \item [] \textbf{()} No
        \end{itemize}
        \item This paper lists all final (hyper-)parameters used for each model/algorithm in the paper’s experiments.
        \begin{itemize}
            \item [] \textbf{(X)} Yes
            \item [] \textbf{( )} Partial
            \item [] \textbf{( )} No
            \item [] \textbf{( )} N/A
        \end{itemize}
        \item This paper states the number and range of values tried per (hyper-)parameter during development of the paper, along with the criterion used for selecting the final parameter setting.
        \begin{itemize}
            \item [] \textbf{()} Yes
            \item [] \textbf{( )} Partial
            \item [] \textbf{( )} No
            \item [] \textbf{(X)} N/A
        \end{itemize}
    \end{enumerate}

\end{enumerate}

